CROSSFIRE: Camera Relocalization On Self-Supervised Features from an Implicit Representation

Beyond novel view synthesis, Neural Radiance Fields are useful for applications that interact with the real world. In this paper, we use them as an implicit map of a given scene and propose a camera relocalization algorithm tailored for this representation. The proposed method enables to compute in real-time the precise position of a device using a single RGB camera, during its navigation. In contrast with previous work, we do not rely on pose regression or photometric alignment but rather use dense local features obtained through volumetric rendering which are specialized on the scene with a self-supervised objective. As a result, our algorithm is more accurate than competitors, able to operate in dynamic outdoor environments with changing lightning conditions and can be readily integrated in any volumetric neural renderer.

==> tables/ablations.tex <==
\begin{minipage}{0.45\columnwidth}
\begin{tikzpicture}[xscale=0.4,yscale=0.4]
        \begin{axis}[major x tick style = transparent,
            ybar,
            ylabel={Test median error},
            ymin=0, ymax=3,
            enlarge x limits=0.5,
            bar width=20pt,
            ymajorgrids = true,
            symbolic x coords={direction dependent,direction independent},
            ytick={0,0.5,1.0,1.5,2.0, 2.5},
            legend pos=north east,
            grid style=dashed,
            xtick = data
        ]
        
        
        \addplot[color=red, fill=red]
            coordinates {(direction dependent,2.2)(direction independent,1.3)};
        
        \addplot[color=cyan, fill=cyan]
            coordinates {
            (direction dependent,0.9)(direction independent,0.4)
            };
            
        \legend{Translation error (cm),Rotation error (°)}
        \end{axis}
\end{tikzpicture}
\captionof{figure}{\textbf{Localization accuracy depending on descriptor head inputs.} We compare the accuracy with and without the viewing direction as descriptor input in the neural renderer.} \label{fig:abl_direction}
\end{minipage}
\hfill
\begin{minipage}{0.45\columnwidth}
\begin{tikzpicture}[xscale=0.4,yscale=0.4]
        \begin{axis}[major x tick style = transparent,
            ybar,
            ylabel={Test median error},
            ymin=0, ymax=3,
            enlarge x limits=0.5,
            bar width=20pt,
            ymajorgrids = true,
            symbolic x coords={MSE+SSIM, MSE+TV,MSE+TV+SSIM},
            ytick={0,0.5,1.0,1.5,2.0, 2.5},
            legend pos=north east,
            grid style=dashed,
            xtick = data
        ]
        
        
        \addplot[color=red, fill=red]
            coordinates {(MSE+SSIM,6.0)(MSE+TV,4.0)(MSE+TV+SSIM, 3.0};
        
        \addplot[color=cyan, fill=cyan]
            coordinates {
            (direction dependent,0.9)(direction independent,0.4)
            };
            
        \legend{Translation error (cm),Rotation error (°)}
        \end{axis}
\end{tikzpicture}
\captionof{figure}{\textbf{Localization accuracy depending on descriptor head inputs.} We compare the final accuracy on the "Chess" scene with and without the viewing direction as descriptor input in the neural renderer.} \label{fig:abl_direction}
\end{minipage}
